Building a Strong Pre-Training Baseline for Universal 3D Large-Scale Perception

An effective pre-training framework with universal 3D representations is extremely desired in perceiving large-scale dynamic scenes. However, establishing such an ideal framework that is both task-generic and label-efficient poses a challenge in unifying the representation of the same primitive across diverse scenes. The current contrastive 3D pre-training methods typically follow a frame-level consistency, which focuses on the 2D-3D relationships in each detached image. Such inconsiderate consistency greatly hampers the promising path of reaching an universal pre-training framework: (1) The cross-scene semantic self-conflict, i.e., the intense collision between primitive segments of the same semantics from different scenes; (2) Lacking a globally unified bond that pushes the cross-scene semantic consistency into 3D representation learning. To address above challenges, we propose a CSC framework that puts a scene-level semantic consistency in the heart, bridging the connection of the similar semantic segments across various scenes. To achieve this goal, we combine the coherent semantic cues provided by the vision foundation model and the knowledge-rich cross-scene prototypes derived from the complementary multi-modality information. These allow us to train a universal 3D pre-training model that facilitates various downstream tasks with less fine-tuning efforts. Empirically, we achieve consistent improvements over SOTA pre-training approaches in semantic segmentation (+1.4% mIoU), object detection (+1.0% mAP), and panoptic segmentation (+3.0% PQ) using their task-specific 3D network on nuScenes. Code is released at https://github.com/chenhaomingbob/CSC, hoping to inspire future research.

==> assets/algorithm.tex <==
% \vspace{4em}
\begin{algorithm}[h]
	\small
	% \setstretch{0.88}
	\caption{Multi-Modality 3D Pre-Training Pipeline for our Coherent Semantic Cues Framework (CSC)}
	\begin{algorithmic}[1]
		\label{alg:algorithm1}
		\STATE \textbf{Input:} (i) the point cloud frame $\boldsymbol{\mathcal{P}}$ and (ii) the surrounding images  $\boldsymbol{\mathcal{I}}$.
		\STATE \textbf{Backbones:} (1) the 2D embedding network $\boldsymbol{\Theta_I}$, (2) the 3D embedding network $\boldsymbol{\Theta_P}$, and (3) the 2D mask network $\boldsymbol{\Theta_F}$.
            \STATE \textbf{Loss:} superpixel-superpoint constrastive loss $\boldsymbol{\mathcal{L}_{\text{sp}}}$ and prototype-based loss $\boldsymbol{\mathcal{L}_{\text{pro}}}$.
		\STATE \textbf{Hyper-parameters:} (a) the starting epoch of using prototype-based loss $\lambda$, (b) the temperature of superpixel-superpoint loss  $\tau_{sp}$, and (c) the temperature of prototype-based loss	 $\tau_{pro}$.		
            \STATE \textbf{Pipeline:}
            \STATE Obtain superpixels $\boldsymbol{\mathcal{S_{\text{2D}}}}$ and semantic cues $\boldsymbol{\mathcal{C}_{\text{sem}}}$ from $\boldsymbol{\mathcal{I}}$ by $\boldsymbol{\Theta_F}$.
            
            \FOR{$n$ in $1$:$MaxEpochs$}
            \IF{$n \bmod \lambda ==0 $}
            \FOR{$i$ in $1$:$iterations$}
            \STATE Extract 2D/3D features from $\boldsymbol{\mathcal{I}}$/$\boldsymbol{\mathcal{P}}$ by $\boldsymbol{\Theta_I}$/$\boldsymbol{\Theta_P}$.
            \STATE According to 2D/3D features, $\boldsymbol{\mathcal{S_{\text{2D}}}}$, and $\boldsymbol{\mathcal{C}_{\text{sem}}}$, to produce the superpixels \& superpoints features $\boldsymbol{\mathcal{F}_{\text{2D}}}$ \& $\boldsymbol{\mathcal{F}_{\text{3D}}}$.
            \STATE Maintain two separate prototype features $\boldsymbol{\mathcal{P}_{\text{2D}}}$ \& $\boldsymbol{\mathcal{P}_{\text{3D}}}$ by $\boldsymbol{\mathcal{F}_{\text{2D}}}$, $\boldsymbol{\mathcal{F}_{\text{3D}}}$, and $\boldsymbol{\mathcal{C}_{\text{sem}}}$.
            \STATE {
            $\boldsymbol{\mathcal{P}_{\text{2D}}} \xrightarrow[]{\text{Linear Layers}} \boldsymbol{\mathcal{\Bar{P}}_{\text{2D}}}$,
            }
            \STATE {
            $\boldsymbol{\mathcal{P}_{\text{3D}}} \xrightarrow[]{\text{Linear Layers}} \boldsymbol{\mathcal{\Bar{P}}_{\text{3D}}}$.
            }
            \STATE {
                $\{\boldsymbol{\mathcal{\Bar{P}}_{\text{2D}}}, \boldsymbol{\mathcal{\Bar{P}}_{\text{3D}}}\} \xrightarrow[]{\text{Linear Layers}} \boldsymbol{\mathcal{P}_{\text{mix}}}$.
            }
            \ENDFOR
            \ENDIF
            
            \FOR{$i$ in $1$:$iterations$}
            \STATE Extract 2D/3D features from $\boldsymbol{\mathcal{I}}$/$\boldsymbol{\mathcal{P}}$ by $\boldsymbol{\Theta_I}$/$\boldsymbol{\Theta_P}$.
            \STATE According to 2D/3D features, $\boldsymbol{\mathcal{S_{\text{2D}}}}$, and $\boldsymbol{\mathcal{C}_{\text{sem}}}$, to generate the superpixels \& superpoints features $\boldsymbol{\mathcal{F}_{\text{2D}}}$ \& $\boldsymbol{\mathcal{F}_{\text{3D}}}$. 
            \STATE  {$\boldsymbol{\mathcal{L}_{\text{sp}}}=-\sum_{i=0}^{Q} \log \frac{\exp \left(\left\langle\boldsymbol{F}_{\text{3D}}^{i}, \boldsymbol{F}_{\text{2D}}^{i}\right\rangle / \tau_{sp}\right)}{\sum_{j=0}^{Q} \exp \left(\left\langle\boldsymbol{F}_{\text{3D}}^i, \boldsymbol{F}_{\text{2D}}^{j}\right\rangle / \tau_{sp}\right)}$}
            
            \IF{$n<\lambda$}
            \STATE {$\boldsymbol{\mathcal{L}_{\text {total}}}=\boldsymbol{\mathcal{L}_{\text{sp}}}$}.
            \ELSE 
            \STATE {$\boldsymbol{\mathcal{L}_{\text{pro}}}=-\log \frac{\exp \left(\left\langle \boldsymbol{F}_{\text{3D}}, \boldsymbol{P}_{\text{mix}}^{+}\right\rangle / \tau_{pro}\right)}{\sum_{i=0}^{|\boldsymbol{\mathcal{C_\text{sem}}}|} \exp \left(\left\langle \boldsymbol{F}_{\text{3D}}, \boldsymbol{P}_{\text{mix}}^{i}\right\rangle / \tau_{pro}\right)}$}.
            \STATE {$\boldsymbol{\mathcal{L}_{\text {total}}}=\boldsymbol{\mathcal{L}_{\text{sp}}}+ \boldsymbol{\mathcal{L}_{\text{pro}}}$}.
            \ENDIF
            \STATE Update $\boldsymbol{\Theta_P}$ by {$\boldsymbol{\mathcal{L}_{\text {total}}}$}.
            \ENDFOR
            \ENDFOR
	\end{algorithmic}
 \label{alg:pseudo_code_pipeline}
\end{algorithm}
% \vspace{2em}

==> figs/distribution_sp_sem.tex <==
\begin{figure*}[h]

\begin{minipage}{.58\linewidth}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/sup_figs/dist_sp_sem_3.png}
\end{minipage}
% \hfill
\hspace{-12mm}
\begin{minipage}{.38\linewidth}
\scalebox{0.8}{
\begin{tabular}{c |c | c}
\toprule
Superpixel Semantic
& Counts
& Percent (\bf \textperthousand{})
\\ 
\midrule
% \tikzmark{start}  
Wall   
& 80.4K
& 88\textperthousand{} 
\\
Grass         
& 75.8K  
& 83\textperthousand{} 
\\
Tree           
& 48.5K  
& 53\textperthousand{} 
\\
Building
& 48.3K  
& 52\textperthousand{} 
\\
Sidewalk      
& 33.9K 
& 37\textperthousand{} 
\\
Railing     
& 10.1K  
& 11\textperthousand{} 
\\ 
Conveyer       
& 4.3K  
& 4\textperthousand{} 
\\
Fence       
& 2.9K  
& 3\textperthousand{} 
\\
Bus       
& 2.8K  
& 3\textperthousand{} 
\\
% \tikzmark{end}
Person
& 2.5K   
& 2\textperthousand{} 
\\
Motorcar
& 110
& 0\textperthousand{} 
\\
Motorbike
& 28   
& 0\textperthousand{} 
\\
\textcolor{gray}{Driving Unrelated Classes}
& \textcolor{gray}{603K}
& \textcolor{gray}{661\textperthousand{} }
\\
\toprule
\end{tabular}
}
\end{minipage}

% \begin{tikzpicture}[overlay, remember picture]
% \draw[red, thick, decorate, decoration={brace, amplitude=10pt, mirror,raise=3pt}]
%   ([yshift=2pt]pic cs:start) -- ([yshift=-2pt]pic cs:end) node [red, midway, yshift=-1.2cm,xshift=-0.8cm, anchor=east,rotate=-90] {OutDoor Classes};
% \end{tikzpicture}

\caption{Semantic classes and number of superpixels generated by DINOV2 on the nuScenes dataset. We provide both the pie chart (left half) and the statistical table (right half) to present the semantic distribution of the superpixels. Note that since we use DINOV2 fine-tuned on the ADE20K dataset \cite{ADE20K}, the network classifies each superpixel in 150 categories, most of which are categories that are unrelated to autonomous driving scenes, such as bed, bench, book, etc. We denote these classes as Driving Unrelated Semantics, which amounted to 603K and accounted for 661\textperthousand{} of the total.}
\label{fig:superpixel_semantic_distribution}
\end{figure*}





==> figs/sup_figs/misclass_from_dinov2.tex <==
\begin{figure}[h]
\centering
\small
\includegraphics[width=1.0\linewidth]{figs/sup_figs/dinov2_misclassfication.pdf}
\vspace{-2.2em}
\caption{
(a) an input image from nuScenes; (b) \colorbox{BlueViolet}{\textcolor{white}{const. veh.}}, \colorbox{DarkCyan}{\textcolor{white}{trailer}} and \colorbox{GoldEnrod}{\textcolor{white}{truck}} in DINOv2; (c) \colorbox{red}{\textcolor{white}{truck}} in nuScenes.
}
\label{fig:dinov2_misclassficaiont}
\end{figure}

==> tables/table2_1pt_semantic_nuscenes.tex <==
\begin{table*}[t]
  \centering
  \setlength{\tabcolsep}{4.0 pt}
  \begin{tabular}{l | l l l l l l l l l l l l l l l l  l }
    \toprule
        \multirow{1}{*}{\bf Method}
        & \multicolumn{1}{R{60}{1em}}{barrier}
        & \multicolumn{1}{R{60}{1em}}{bicycle}
        & \multicolumn{1}{R{60}{1em}}{bus}
        & \multicolumn{1}{R{60}{1em}}{car}
        & \multicolumn{1}{R{60}{1em}}{const. veh.}
        & \multicolumn{1}{R{60}{1em}}{motorcycle}
        & \multicolumn{1}{R{60}{1em}}{pedestrian}
        & \multicolumn{1}{R{60}{1em}}{traffic cone}
        & \multicolumn{1}{R{60}{1em}}{trailer}
        & \multicolumn{1}{R{60}{1em}}{truck}
        & \multicolumn{1}{R{60}{1em}}{driv. surf.}
        & \multicolumn{1}{R{60}{1em}}{other flat}
        & \multicolumn{1}{R{60}{1em}}{sidewalk}
        & \multicolumn{1}{R{60}{1em}}{terrain}
        & \multicolumn{1}{R{60}{1em}}{manmade}
        & \multicolumn{1}{R{60}{1em}}{vegetation}
        & \multicolumn{1}{R{60}{1em}}{\bf mIoU}
        \\
    \midrule
        Random Init. 
        & 0.0
        & 0.0
        & 8.1
        & 65.0
        & 0.1
        & 6.6
        & 21.0
        & 9.0
        & 9.3
        & 25.8
        & 89.5
        & 14.8
        & 41.7
        & 48.7
        & 72.4
        & 73.3
        & 30.3
        \\
        Point Con. \cite{xie2020pointcontrast}
        & 0.0
        & 1.0
        & 5.6
        & 67.4
        & 0.0
        & 3.3
        & 31.6
        & 5.6
        & 12.1
        & 30.8
        & 91.7
        & 21.9
        & 48.4
        & 50.8
        & 75.0
        & 74.6
        & 32.5
        \\
        Depth Con. \cite{zhang2021self}
        & 0.0
        & 0.6
        & 6.5
        & 64.7
        & 0.2
        & 5.1
        & 29.0
        & 9.5
        & 12.1
        & 29.9
        & 90.3
        & 17.8
        & 44.4
        & 49.5
        & 73.5
        & 74.0
        & 31.7
        \\
        SLidR \cite{sautier2022image}
        & 0.0
        & 3.1
        & 15.2
        & 72.0
        & 0.9
        & 18.8
        & 43.2
        & 12.5
        & 14.7
        & 33.3
        & 92.8
        & 29.4
        & 54.0
        & 61.0
        & 80.2
        & 81.9
        & 38.3
        \\
        ST-SLidR \cite{mahmoud2023self}
        & 0.0
        & 2.7
        & 16.0
        & 74.5
        & 3.2
        & 25.4
        & 50.9
        & 20.0
        & 17.7
        & 40.2
        & 92.0
        & 30.7
        & 54.2
        & 61.1
        & 80.5
        & 82.9
        & 40.7
        \\
        TriCC \cite{pang2023unsupervised}
        & 0.0
        & 2.6
        & 20.7
        & 73.6
        & 0.3
        & 18.9
        & 49.2
        & 22.0
        & 16.9
        & 33.4
        & \bf 94.5
        & 43.1
        & 57.2
        & 62.1
        & 82.3
        & 82.6
        & 41.2
        \\
        Seal \cite{liu2023segment}
        & 0.0
        & \bf 9.4
        & 32.6
        & \bf 77.5
        & \bf 10.4
        & 28.0
        & 53.0
        & 25.0
        & \bf 30.9
        & \bf 49.7
        &  94.0
        & \bf 33.7
        & \bf 60.1
        & 59.6
        & \bf 83.9
        & 83.4
        & 45.8
        \\
    % \midrule
        \rowcolor{gray!20}
        Ours
        & 0.0
        & 0.0
        & \bf 58.7
        & 74.0
        & 0.1
        & \bf 40.9
        & \bf 58.9
        & \bf 31.8
        & 23.7
        & 45.1
        & 92.5
        & 33.0
        & 56.4
        & \bf 62.4
        & 81.6
        & \bf 84.2
        & \bf 47.0
        \\
    \bottomrule
  \end{tabular}
  \caption{Per-class IoU on nuScenes  when fine-tunning with 1\% labels }
  \label{tab:1pt_sem_seg}
\end{table*}

==> tables/table5_unsupervised_semseg.tex <==
\begin{table}[t]
\centering      
\scalebox{0.9}{
\begin{tabular}{l| c | c c }        
        \toprule        
        \multirow{2}{*}{\bf Method} 
        & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Involved} \\ \textbf{Modalities}\end{tabular}} 
        &  \multicolumn{2}{c}{\bf nuScenes}
        \\    
        \cline{3-4}
        {}
        & {}
        &  mAcc
        &  mIoU
        \\
        \midrule 
        \multicolumn{3}{l}{\textit{Fully-supervised methods}} 
        \\
        MinkUNet \cite{choy20194d}
        & P
        & 0.0
        & 74.2
        \\
        VoXelNet  \cite{zhou2018voxelnet}
        & P
        & 0.0
        & 0.0
        \\  
        Cylinder3D \cite{cylinder3d}
        & P
        & 0.0
        & 0.0
        \\ 
        \bottomrule    
        \multicolumn{3}{l}{\textit{Zero-shot methods}}
        \\
        MSeg Voting \cite{mseg}
        & P
        &36.9
        &31.0 
        \\
        CLIP2Scene \cite{clip2scene}
        & P,{\ }C,{\ }T
        &-
        &20.8
        \\ 
        OpenScene \cite{openscene} - LSeg \cite{Lseg}
        & P,{\ }C,{\ }T
        &36.7
        &42.7 
        \\ 
        OpenScene \cite{openscene} - OpenSeg \cite{openseg}
        & P,{\ }C,{\ }T
        &61.8 
        &42.1
        \\  
        \rowcolor{gray!20}
        Ours
        & P,{\ }C
        &\textbf{0.0}
        &\textbf{0.0}
        \\ 
        \rowcolor{gray!20}
        Ours - OneFormer \textsuperscript{\textdagger}
        & P,{\ }C
        &\textbf{0.0}
        &\textbf{0.0}
        \\ 
        \rowcolor{gray!20}
        Ours - OneFormer \textsuperscript{\textdaggerdbl}
        & P,{\ }C
        &\textbf{0.0}
        &\textbf{0.0}
        \\ 
        \bottomrule 
\end{tabular} 
}
\caption{Caption}
\label{tab:ann_free_sem_seg}
\end{table} 


